Boosting Semi-Supervised Temporal Action Localization by Learning from Non-Target Classes

The crux of semi-supervised temporal action localization (SS-TAL) lies in excavating valuable information from abundant unlabeled videos. However, current approaches predominantly focus on building models that are robust to the error-prone target class (i.e, the predicted class with the highest confidence) while ignoring informative semantics within non-target classes. This paper approaches SS-TAL from a novel perspective by advocating for learning from non-target classes, transcending the conventional focus solely on the target class. The proposed approach involves partitioning the label space of the predicted class distribution into distinct subspaces: target class, positive classes, negative classes, and ambiguous classes, aiming to mine both positive and negative semantics that are absent in the target class, while excluding ambiguous classes. To this end, we first devise innovative strategies to adaptively select high-quality positive and negative classes from the label space, by modeling both the confidence and rank of a class in relation to those of the target class. Then, we introduce novel positive and negative losses designed to guide the learning process, pushing predictions closer to positive classes and away from negative classes. Finally, the positive and negative processes are integrated into a hybrid positive-negative learning framework, facilitating the utilization of non-target classes in both labeled and unlabeled videos. Experimental results on THUMOS14 and ActivityNet v1.3 demonstrate the superiority of the proposed method over prior state-of-the-art approaches.

==> Tables/I3D-backbone2.tex <==
\begin{table}[t]
	\centering
	\resizebox{.5\linewidth}{!}{
		\setlength{\tabcolsep}{0.55em}%
		\begin{tabular}{c|c|ccc}
			\toprule %\hline
			\specialrule{0em}{1.0pt}{1.0pt}
			\multirow{2}{*}{Labels} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{THUMOS14 (\%)} \\
			\cmidrule{3-5}
			& & 0.3  & 0.5  & 0.7 \\ 
			\midrule % \hline
			\multirow{4}{*}{10\%}
			& SSP~\cite{ji2019learning} & 43.1 & 25.5 & 9.6\\
			& SSTAP~\cite{wang2021self} & 45.3 & 27.5 & 11.0\\
			& SPOT~\cite{nag2022semi} & 49.1 & 31.7 & 12.6 \\
			& Ours & \textbf{51.3} & \textbf{34.8} & \textbf{14.9} \\
			\midrule
			\multirow{4}{*}{60\%}
			& SSP~\cite{ji2019learning} & 53.5 & 39.7 & 20.4\\
			& SSTAP~\cite{wang2021self} & 55.9 & 41.6 & 22.0\\
			& SPOT~\cite{nag2022semi} & 58.7 & 42.4 & 23.1 \\
			& Ours & \textbf{59.8} & \textbf{44.1} & \textbf{24.3} \\
			\bottomrule 
		\end{tabular}
	}
	\caption{\textbf{SS-TAL results using I3D features} on THUMOS14, where we use 10\% and 60\% labeled data.}
	\label{tab:ablation-on-i3d}
\end{table}
% in terms of mAP~(\%)

==> Tables/effectiveness-of-components-anet.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.6\linewidth}{!}{
		\setlength{\tabcolsep}{0.65em}%
		\begin{tabular}{ccc|cccc}
			\toprule %\hline
			\specialrule{0em}{1.0pt}{1.0pt}
			\multirow{2}{*}{$\ell^{tgt}$} & \multirow{2}{*}{$\ell^{neg}$} & \multirow{2}{*}{$\ell^{pos}$}& \multicolumn{4}{c}{ActivityNet v1.3 (\%)} \\
			\cmidrule{4-7}
			& & & 0.5  & 0.75  & 0.95 & Avg. \\ 
			\midrule % \hline
			\Checkmark &  & & 51.2 & 31.8 & 7.3 & 32.1    \\
			\Checkmark  & \Checkmark  & & 52.3 & 32.7  & 8.3 &  33.4 \\
			\Checkmark   & \Checkmark & \Checkmark & \textbf{53.0} & \textbf{34.4} & \textbf{9.2} & \textbf{34.5}    \\
			\bottomrule 
		\end{tabular}
	}
	\caption{Ablation study of different losses on ActivityNet v1.3 with 10\% labels, where $\ell^{tgt}$ is the vanilla cross-entropy loss for snippet-level action classification, and $\ell^{neg}$ and $\ell^{pos}$ are the proposed negative and positive learning losses for excavating complementary information.}
	\label{tab:ablation-on-anet}
\end{table}
% in terms of mAP~(\%)

==> Tables/hyperparameters.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.5\linewidth}{!}{
		\setlength{\tabcolsep}{0.65em}%
		\begin{tabular}{c|cccc}
			\toprule %\hline
			\specialrule{0em}{1.0pt}{1.0pt}
			\multirow{2}{*}{$\lambda$ value} & \multicolumn{4}{c}{THUMOS14 (\%)} \\
			\cmidrule{2-5}
			& 0.3  & 0.5  & 0.7 & Avg. \\ 
			\midrule % \hline
			0.90 & 50.6 & 34.8 &  14.3 & 33.2\\
			0.85 & \textbf{50.9} & \textbf{34.9} & \textbf{14.6} & \textbf{33.5} \\
			0.80 & 50.2 & 34.3 & 14.1 & 33.0  \\
			\bottomrule 
		\end{tabular}
	}
	\caption{Empirical study of hyper-parameter $\lambda$ on THUMOS14 with 10\% labels, where $\lambda$ affects the number of the positive classes for positive learning.}
	\label{tab:ablation-on-lambda}
\end{table}
% in terms of mAP~(\%)

==> Tables/label-space.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.6\linewidth}{!}{
		\setlength{\tabcolsep}{0.75em}%
		\begin{tabular}{c|c|c|c}
			\toprule %\hline
			\specialrule{0em}{1.0pt}{1.0pt}
			$\Omega^{tgt}$ & $\Omega^{pos}$ & $\Omega^{amb}$ & $\Omega^{neg}$ \\
			\midrule % \hline
			19.4 & 59.7 & 18.5 & 2.4\\
			\bottomrule 
		\end{tabular}
	}
	\caption{The average probability that the ground truth label is located in different sets, \textit{i.e.} target class set $\Omega^{tgt}$, positive class set $\Omega^{pos}$, ambiguous class set $\Omega^{amb}$ and negative class set $\Omega^{neg}$. The experiment is performed on 90\% unlabeled videos on THUMOS14.}
	\label{tab:ablation-on-prob}
\end{table}
% in terms of mAP~(\%)
